Value Iteration Networks

We introduce the value iteration network (VIN): a fully differentiable neural network with a `planning module' embedded within. VINs can learn to plan, and are suitable for predicting outcomes that involve planning-based reasoning, such as policies for reinforcement learning. Key to our approach is a novel differentiable approximation of the value-iteration algorithm, which can be represented as a convolutional neural network, and trained end-to-end using standard backpropagation. We evaluate VIN based policies on discrete and continuous path-planning domains, and on a natural-language based search task. We show that by learning an explicit planning computation, VIN policies generalize better to new, unseen domains.

==> old_stuff.tex <==
\subsection{Problem Formulation}
We consider a structured prediction \citep{bakir2007predicting,nowozin2011structured} problem in which the input consists of a dataset of images $\left\{x^i\right\}_{i=1,\dots,N}$, states $\left\{s^i\right\}_{i=1,\dots,N}$, and action labels $\left\{ a^i \right\}_{i=1,\dots,N}$. We assume that the actions are generated from an optimal policy $a^i = \pi^*(s^i)$ with respect to some unknown MDP, encoded in the image $x^i$. For example, in the path planning domains we consider, the state $s$ encodes the position, and the image shows the obstacles and a goal location. The action then encodes the direction of the shortest path to the goal between the obstacles. We emphasize that the reward and transitions in the MDP are unknown, and are not an explicit part of the input in any way.

Our goal is to learn a mapping $y(x,s)$ that best predicts the correct action label for an image and state. 
\Naively, this problem can be cast as a standard supervised learning problem \cite{Bishop2006}, by concatenating $x$ and $s$ into a single observation. With enough training data, it is conceivable that a standard supervised learning algorithm would learn a suitable solution. However, such a \naive\ approach ignores the knowledge about the process that generates the data. By exploiting this knowledge, a solution may be found more efficiently. In the following, we propose a class of neural network representations that incorporate a `planning module' in their structure. We shall show that this structure enables much more efficient learning than standard feed-forward networks in this problem domain.

\begin{table}
\begin{center}
  \begin{tabular}{ | c | c | c | c | c | c | c | c | c | c |}
    \hline
    \multirow{2}{*}{Domain} 
    & \multicolumn{3}{|c|}{VIN} 
    & \multicolumn{3}{|c|}{Hierarchical VIN} 
    & \multicolumn{3}{|c|}{1-layer FC} \\ \cline{2-10}
     & Prediction & Success & Trajectory 
     & Pred. & Succ. & Traj. 
     & Pred. & Succ. & Traj. \\ 
     & loss & rate & difference 
     & loss & rate & diff. 
     & loss & rate & diff. \\ \hline 

    $8 \times 8$ & \bf 0.004 & \bf 99.6\% & 0.001 
    & 0.005 & 99.3\% & \bf 0.0 
    & 0.08 & 80.6\% & 0.001 \\ \hline 
    $16 \times 16$ & 0.05 & \bf 99.3\% & 0.089 
    & \bf 0.03 & 99\% & \bf 0.007 
    & 0.25 & 54.4\% & 0.14 \\ \hline 
    $28 \times 28$ & 0.11 & 97\% & 0.086 
    & \bf 0.05 & \bf 98.1\% & \bf 0.037 
    & 0.40 & 7.1\% & 0.80 \\ \hline 
    $36 \times 36$ & 0.14 & 92.3\% & 0.21 
    & \bf 0.09 & \bf 93.8\% & \bf 0.14 
    &  &  & \\ \hline 
  \end{tabular}

\vspace{10pt}

  \begin{tabular}{ | c | c | c | c | c | c | c | c | c | c |}
    \hline
    \multirow{2}{*}{Domain} 
    & \multicolumn{3}{|c|}{2-layer FC} 
    & \multicolumn{3}{|c|}{CNN} 
    & \multicolumn{3}{|c|}{FCN} \\ \cline{2-10}
     & Pred. & Succ. & Traj. 
     & Pred. & Succ. & Traj. 
     & Pred. & Succ. & Traj.\\ 
     & loss & rate & diff. 
     & loss & rate & diff. 
     & loss & rate & diff.\\ \hline 

    $8 \times 8$ & 0.08 & 82.8\% & 0.004 
    & 0.02 & 97.9\% & 0.006 
    & 0.01 & 97.3\%& 0.004\\ \hline 
    $16 \times 16$ & 0.24 & 55.8\% & 0.07 
    & 0.10 & 87.6\% & 0.06 
    & 0.07 & 88.3\% & 0.05 \\ \hline 
    $28 \times 28$ & 0.35 & 22.1\% & 0.62 
    & 0.13 & 74.2\% & 0.078 
    & 0.09 & 76.6\% & 0.08 \\ \hline 
  \end{tabular}
  
\vspace{10pt}

  \begin{tabular}{ | c | c | c | c | c | c | c | c | c | c |}
    \hline
    \multirow{2}{*}{Training data} 
    & \multicolumn{3}{|c|}{VIN} 
    & \multicolumn{3}{|c|}{VIN Untied Weights} 
    & \multicolumn{3}{|c|}{} \\ \cline{2-10}
     & Pred. & Succ. & Traj. 
     & Pred. & Succ. & Traj. 
     & Pred. & Succ. & Traj.\\ 
     & loss & rate & diff. 
     & loss & rate & diff. 
     & loss & rate & diff.\\ \hline 

    $20\%$ & 0.06 & 98.2\% & 0.106 & 0.09 & 91.9\% & 0.094 & & & \\ \hline 
    $50\%$ & 0.05 & 99.4\% & 0.018 & 0.07 & 95.2\% & 0.078 &  & \% &  \\ \hline 
    $100\%$ & 0.05 & 99.3\% & 0.089 & 0.05 & 95.6\% & 0.068 &  & \% &  \\ \hline 
  \end{tabular}
  
  
  %\paragraph{Hierarchical VIN network}
%We used the hierarchical VIN model of Section \ref{ss:MultiResVIN}, with a $2 \times 2$ down-sampling layer. Similarly to the VI network, we used $3 \times 3$ convolution kernels, $150$ channels for each hidden layer $H$ (for both the down-sampled image, and standard image), and $10$ channels for the $q$ layer in each VI block. Similary to the VIN networks, the recurrence $K$ was set relative to the problem size, taking into account the down-sampling factor: $K=4$ for $8 \times 8$ domains, $K=10$ for $16 \times 16$ domains, $K=16$ for $28 \times 28$ domains, and $K=20$ for $36 \times 36$ domains. 
%\paragraph{Fully-connected feed-forward network}
%In order to train a standard multi-layer fully-connected (FC) feed-forward network (also known as a multi-layer perceptron model), we flattened out the obstacle and goal images, and represented the state $(i,j)$ as two 1-hot vectors (a vector for each coordinate), for a total of $2 \times m \times n + m + n$ inputs. We constructed both a single hidden-layer FC network, with 256 hidden units, and a two-layer FC network, with 256 hidden units in each hidden layer, and ReLU non-linearity. The number of hidden units was chosen by trial and error.
%\paragraph{Feed-forward CNN}
%This model is an extension of the single layer FC network, in which the input images are first fed into 2 convolution layers, with $3\times 3$ convolution kernels, $8$ and $16$ channels, respectively, and $2 \times 2$ max-pooling. The output of these layers, along with the 1-hot state vectors, are fed into a single hidden-layer FC network, with 256 hidden units.

==> related.tex <==
Learning to predict trajectories is an instance of structured prediction problems \citep{bakir2007predicting,nowozin2011structured}. In particular, structured prediction strategies such as maximum-margin prediction \citep{ratliff2006maximum} have been applied to imitation learning of trajectories from demonstrations. In this setting, the transitions in the MDP underlying the planning process are assumed to be known, but the cost has to be learned from data. A similar approach is also used in inverse reinforcement learning (IRL) \citep{abbeel2004apprenticeship,ziebart2008maximum,levine2011nonlinear}, which has been used for similar domains of predicting trajectories from overhead images as in this work \cite{kitani2012activity,ratliff2009learning}. Our approach is somewhat orthogonal to these methods, as we encode the planning process directly in our policy, relieving the need to use specialized learning algorithms that exploit the underlying MDP. To emphasize this point, in this work we trained our models using a standard classification-learning algorithm. However, our approach can be easily incorporated within a no-regret structured prediction method such DAgger \cite{ross2011reduction} to potentially yield improved results. We remark that although we do not explicitly use a model, the local convolutions applied in our networks do exploit some structure of the underlying MDP. However, this prior knowledge is still considerably less than knowing the exact transitions. 

Similar to our approach, \citet{zucker2012reinforcement} suggested gradient-based approaches for learning better planners. In that work, a linearly parameterized cost function was learned using reinforcement-learning techniques. In a different study, \citet{singh2010intrinsically} used evolutionary algorithms to learn a cost function that accelerates learning. Our work is substantially different, in learning both costs and transitions of an approximate planning algorithm, and using highly expressive neural networks instead of linear function approximators. 

Another relevant line of work is the recent trend of approximating algorithms using neural networks, such as the neural turing machines \citep{graves2014neural}, pointer networks \citep{vinyals2015pointer}, and the recurrent networks of \citet{zaremba2015learning}. Our approach can be seen as a neural-network approximation of dynamic programming (VI), learned from examples.

